Dynamic Distribution State Estimation Using Synchrophasor Data

The increasing deployment of distribution-level phasor measurement units (PMUs) calls for dynamic distribution state estimation (DDSE) approaches that tap into high-rate measurements to maintain a comprehensive view of the distribution-system state in real time. Accordingly, this paper explores the development of a fast algorithmic framework by casting the DDSE task within the time-varying optimization realm. The time-varying formulation involves a time-varying robustified least-squares approach, and it naturally models optimal trajectories for the estimated states under streaming of measurements. The formulation is based on a linear surrogate of the AC power-flow equations, and it includes an element of robustness with respect to measurement outliers. The paper then leverages a first-order prediction-correction method to achieve simple online updates that can provably track the state variables from heterogeneous measurements. This online algorithm is computationally efficient as it relies on the Hessian of the cost function without computing matrix-inverse. Convergence and bounds on the estimation errors of proposed algorithm can be analytically established.

==> Results.tex <==
\section{Case Studies}
\label{sec:results}
\begin{figure} [b!!]
	\centering
	%\includegraphics[width = 0.75\linewidth]{Figs/WSCC/WSCC.pdf}
	\epsfig{file = Figs/WSCC_SauerDampCoeff/Oneline.eps, width = 1\linewidth}
	\caption{One-line diagram of the WSCC test case \cite{milano2005psat}.}
	\label{fig:WSCConeline}
\end{figure}

\begin{figure*}[t!!!]
	\centering
	\epsfig{file = Figs/WSCC_SauerDampCoeff/WSCC1.eps, width = \linewidth}
	\caption{Comparison of model-based and estimated frequency response for the WSCC test case with classical generator model and under uniform damping condition.}
	\label{fig:WSCC}
\end{figure*}

This section validates the proposed algorithm using synthetic data generated by the WSCC test case and real synchrophasor data collected at the Eastern Interconnection (EI) system. The synthetic data tests demonstrate the validity of our approach even if (as1)-(as3) fail to hold in practice, including non-symmetric $\bbK$,  non-uniform damped modes, and higher-order generator dynamic model. Real data tests can verify the proposed method's capability in estimating the propagation time of frequency disturbance across the EI system. Since the scaling factor in [S4] requires the knowledge of actual system frequency nadir, the validations will not account for this step. Instead, the following normalized dissimilarity score is used:
\begin{align}
S_{\ell k} = \frac{\|\bar T_{\ell k} - \bar{C}_{\ell k}\|_2}{\|\bar T_{\ell k}\|_2} \label{equ:disscore}
\end{align}
where $\bar T_{\ell k}$ ($\bar {C}_{\ell k}$) stands for the model-based (estimated) response normalized by its maximum absolute value, while $\|\cdot\|_2$ stands for the $L^2$ norm of a function. The normalized metric is effective for comparing the shape of the two time series. An almost zero $S_{\ell k}$ implies that the cross-correlation can accurately recover a scaled version of $T_{\ell k}$, while a higher value of $S_{\ell k}$ indicates a larger mismatch.

\subsection{WSCC Case with Classical Generator Model}

\label{sec:wsccclass}
We use the WSCC 3-generator test case under the classical generator model with the parameters given by \cite{milano2005psat}. A one-line diagram of this system is shown in Fig. \ref{fig:WSCConeline}. Generators at buses 1, 2 and 3 are indexed by the associated bus number. First consider a uniformly-damped system satisfying (as2) with $\gamma = 0.2$; i.e., $D_i = 0.2M_i$ for $i=1,2,3$. Synthetic ambient frequency data are generated using two methods: i) linearized model based on the system \eqref{equ:linearizedmodel}, and ii) time-domain simulation for the non-linear DAEs in \eqref{equ:DAEs}. All the data computations are performed in the Matlab$^\circledR$ environment.

For the linearized model method, matrices $\bbM$, $\bbK$ and $\bbD$ in \eqref{equ:linearizedmodel} are first computed by the PSAT software \cite{milano2005psat}. Accordingly, the system state-space form can be easily constructed while  ambient frequency deviation samples can be formed by simulating the system (using the $lsim$ command) in response to the random input $\bbu$ generated by the $randn$ function. Note that the resultant $\bbK$ is not perfectly symmetric as asserted in (as1) because the transmission lines are not purely inductive. Nonetheless, the line resistance-to-reactance (R/X) ratio is very small almost everywhere, and thus $\bbK$ is nearly symmetric. The highest R/X ratio has been observed to be around 20\% for the lines connecting buses (5,7), and (4,6). The R/X ratio for the other lines is around 12\%. As both lines (5,7) and (4,6) are connecting the generator at bus 1 to other buses, it has been observed that the asymmetry of $\bbK$ is slightly more evident at entries corresponding to bus 1. %To synthesize  ambient frequency data, one can simulate the system response (using the $lsim$ command) to the random input $\bbu$ generated by the $randn$ function. 

Despite of an asymmetric  $\bbK$ violating (as1), we observe that the estimated $\bar {C}_{\ell k}$ matches very well with the model-based result. %The computation is done in Matlab with the system in \eqref{equ:linearizedmodel} converted to state-space form using the $ss$ command. 
Based on the linearized model, the actual frequency response can be calculated using the $impulse$ command, 
%To generate ambient responses, we synthesize the white-noise input using the $randn$ command and simulate the system response using the $lsim$ command. 
while the discrete-time $\bar {C}_{\ell k}$ is obtained based on \eqref{equ:xcordef} of [S3]. Fig. \ref{fig:WSCC} plots the comparisons between the model-based frequency response (in solid red lines) and the estimated one (in dashed blue lines), both normalized by the respective maximum absolute value, for each input-output pair. It has illustrated the high accuracy of the proposed algorithm in recovering the actual time series. This observation has also been corroborated by Table \ref{tbl:WSCC}, which lists the corresponding dissimilarity scores as defined by \eqref{equ:disscore}. The score values are all very close to zero, with slightly higher values related to the generator at bus 1; e.g., between the pairs ($u_1$, $\omega_2$), ($u_1$, $\omega_3$), ($u_2$, $\omega_1$) and ($u_3$, $\omega_1$). These relatively higher mismatches could be related to the earlier observation that the asymmetry of $\bbK$ is more significantly affected at entries corresponding to generator 1.

\begin{table}[]
	\centering
	\caption{Dissimilar scores for the WSCC test case under uniform damping condition}
	\label{tbl:WSCC}
	\begin{tabular}{cccccccccc}
		& \multicolumn{4}{c}{Linearized model}                                                                                   &                       & \multicolumn{4}{c}{Time-domain simulation}                                                                                    \\ \cline{2-5} \cline{7-10} 
		\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{$u_1$} & \multicolumn{1}{c|}{$u_2$} & \multicolumn{1}{c|}{$u_3$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{$u_1$} & \multicolumn{1}{c|}{$u_2$} & \multicolumn{1}{c|}{$u_3$} \\ \cline{2-5} \cline{7-10} 
		\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{$\omega_1$} & \multicolumn{1}{c|}{0.035} & \multicolumn{1}{c|}{0.059} & \multicolumn{1}{c|}{0.039} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\omega_1$} & \multicolumn{1}{c|}{0.113} & \multicolumn{1}{c|}{0.259} & \multicolumn{1}{c|}{0.183} \\ \cline{2-5} \cline{7-10} 
		\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\omega_2$} & \multicolumn{1}{c|}{0.053} & \multicolumn{1}{c|}{0.036} & \multicolumn{1}{c|}{0.030} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\omega_2$} & \multicolumn{1}{c|}{0.249} & \multicolumn{1}{c|}{0.332} & \multicolumn{1}{c|}{0.226} \\ \cline{2-5} \cline{7-10} 
		\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\omega_3$} & \multicolumn{1}{c|}{0.047} & \multicolumn{1}{c|}{0.033} & \multicolumn{1}{c|}{0.017} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\omega_3$} & \multicolumn{1}{c|}{0.180} & \multicolumn{1}{c|}{0.229} & \multicolumn{1}{c|}{0.158} \\ \cline{2-5} \cline{7-10} 
	\end{tabular}
\end{table}

\begin{figure*}[ht!]
	\centering
	\epsfig{file = Figs/WSCC_SauerDampCoeff/WSCC_nonunidamp1.eps, width = \linewidth}
	\caption{Comparison of model-based and estimated frequency response for the WSCC test case with classical generator model and under non-uniform damping condition.}
	\label{fig:WSCCnonunidamp}
\end{figure*}

\subsection{WSCC Case with Higher-order Generator Model}
\begin{figure*}[t]
	\centering
	\epsfig{file = Figs/WSCC_SauerDampCoeff/WSCC_TG_Ex_PSS_6thOrder1.eps, width = \linewidth}
	\caption{Comparison of model-based and estimated frequency response for the WSCC test case with sixth-order generator model and under uniform damping condition.}
	\label{fig:WSCCfull}
\end{figure*}


\begin{table}[tb!]
	\centering
	\caption{Dissimilar scores for the WSCC test case under non-uniform damping condition}
	\label{tbl:WSCCnonunidamp}
	\begin{tabular}{|c|c|c|c|}
		\hline
		& $u_1$ & $u_2$ & $u_3$ \\ \hline
		$\omega_1$ & 0.095 & 0.182 & 0.191 \\ \hline
		$\omega_2$ & 0.177 & 0.172 & 0.311 \\ \hline
		$\omega_3$ & 0.197 & 0.315 & 0.208 \\ \hline
	\end{tabular}
\end{table}

Moreover, we have used time-domain simulation based on the original non-linear model \eqref{equ:DAEs} to generate ambient frequency samples. This data generation method can more accurately represent real system responses by accounting for the non-linearity of power flow equations. However, it is also much more time consuming compared to the earlier method because of the numerical integration computations.  We have slightly modified the integration module routine  $pert.m$  in PSAT \cite{milano2005psat} to incorporate  white-noise perturbation as the generator power input. The noise covariance matrix is set to be $\bbSigma = 0.001\bbM$. Note that this method does not produce the generator speed deviation in the synchronous reference frame, but instead the actual values at around 60Hz. Hence, the output speed data need to be detrended to obtain the ambient deviation from nominal value. Subtracting the output from its time-averaged value serves this purpose well, because the system is slightly perturbed at a single operating point. By cross-correlating the detrended outputs, we plot the estimated frequency response in Fig. \ref{fig:WSCC} using dash-dot green lines, along with the updated dissimilar scores included in Table \ref{tbl:WSCC}. In general, the effectiveness of the cross-correlation approach has been validated by the time-domain simulation output, with slightly increased dissimilarity scores compared to those obtained by the linearized model outputs. But still, the estimated frequency response can well approximate the model-based one, especially at the first few seconds when higher level of amplitude would occur as shown by Fig. \ref{fig:WSCC}. Similar to the validation results using linearized model outputs, relatively higher level of dissimilarity has been observed for the input-output pairs associated with generator 1, particularly for the pairs ($u_1$, $\omega_2$) and ($u_2$, $\omega_1$). This observation can be again attributed to the transmission line $(5,7)$ at high R/X ratio. Since the time-domain simulation method has shown similar estimation/validation results as the linearized model one, we would only use the latter method which allows to very quickly generate  ambient speed data.

We further test the applicability of the proposed approach by relaxing the uniform damping assumption in (as2). All the models and parameters stay the same, except that the damping coefficient for each generator is changed as follows: $D_1 = 0.1 M_1$, $D_2 = 0.2 M_2$ and $D_3 = 0.3 M_3$; see \cite[pp. 165]{sauer1997power}. Under this setting, the damping coefficient for each oscillation mode is 0.279, 0.186, or 0.269, respectively, compared to the 0.2 value for all modes in the uniformly damped case.  Fig. \ref{fig:WSCCnonunidamp} updates the comparison of frequency response, while the corresponding dissimilarity scores are listed in Table \ref{tbl:WSCCnonunidamp}. Compared to the uniformly damped results using linearized model outputs, the dissimilarity score has increased, especially for the pairs $(u_2,\omega_3)$ and $(\omega_3, u_2)$. A closer look at the corresponding curves in Fig. \ref{fig:WSCCnonunidamp} shows a scaling difference in peak values. Under non-uniform damping, the $\bbM$-orthogonality condition in \eqref{equ:Morth} no longer holds, and thus the cross-correlation in \eqref{equ:xcorij} would involve inter-mode components and the coefficients would not match with the model-based analysis. Accordingly, the peak scaling cannot be accurately recovered. Nonetheless, Fig. \ref{fig:WSCCnonunidamp} still shows that the peak locations are well aligned between the estimated and actual ones. This observation sheds light on the applicability of the proposed approach in estimating disturbance propagation time under non-uniform damping scenarios. 






\begin{figure*}[t]
	\centering
	\epsfig{file = Figs/WSCC_SauerDampCoeff/WSCC_TG_Ex_PSS_6thOrder_NonUniformDamp1.eps, width = \linewidth}
	\caption{Comparison of model-based and estimated frequency response for the WSCC test case with sixth-order generator model and under non-uniform damping condition.}
	\label{fig:WSCCfull_nonunidamp}
\end{figure*}

To make the validation more realistic, we modify the WSCC case using the sixth-order generator model that includes controllers like exciter, governor, and power system stabilizer. This modified system is tested under similar settings as in Sec. \ref{sec:wsccclass}. The updated plots for uniform and non-uniform damping conditions are shown in Figs. \ref{fig:WSCCfull} and \ref{fig:WSCCfull_nonunidamp}, respectively. The mismatch of the cross-correlation estimates has become further noticeable, especially in the peak scaling. This is again due to the violation of the ideal (as1)-(as2), in particular the orthogonality condition. It is also observed that the modes are better damped with the additional controllers. Interestingly,  the estimated response has correctly reflected this improvement in damping as the match in the curvature shape is very perfect. As a result, the estimated response has an accurate peak timing alignment, which confirms the applicability of the proposed approach in estimating disturbance propagation time from real power system frequency measurements. % corresponding FDR, their peak locations are aligned in time, as in  Additional damping provided by the controllers (the oscillations in Figs. \ref{fig:WSCCfull} and \ref{fig:WSCCfull_nonunidamp} are damped much faster than the ones in Figs. \ref{fig:WSCC} and \ref{fig:WSCCnonunidamp}) violates assumption \as{2} being violated. For this reason, cross correlation is no longer an exact scaled version of the FDR. Nevertheless, similar to the non-uniformly damped test case, the first peak locations of the FDR and the cross correlation are aligned in time. The peak locations alignment observation thus opens the opportunity to estimate the frequency disturbance propagation time on real power systems, i.e., how long it would take for one location to see the effect of frequency disturbance at another location.

\subsection{Real Data Test}
\label{subsec:realmeas}

We apply the cross-correlation method to real ambient frequency measurements at the Eastern Interconnection (EI) system to estimate its frequency response behavior. The data was collected by the frequency monitoring network (FNET) devices for 15min on January 20, 2017, at a 10Hz sampling rate. Measurement locations include places in the Midwest, South, and Northeast regions. The proposed cross-correlation result is compared with the recorded response during the 2008 Florida blackout. \colorcode{This event is among the most recent wide-area disturbances affecting an interconnected system, and thus can serve as a good reference for validating the effectiveness of our proposed data-driven approach.} %, Mismatch between the estimated frequency responses using data in 2017 and the recorded ones in 2008 is expected due to various reasons, as explained at the end of this sub-section. Nevertheless, this comparison verifies the applicability of the proposed method in an actual wide-area interconnected system.}

The 2008 Florida blackout was caused by a load switching disturbance propagated across the whole EI footprint in the afternoon of February 26, 2008 \cite{liu2016wamsystem}. This event can be approximated by an impulse input to a Florida substation at 18:09:8.2 UTC. \colorcode{Replay of the frequency response and its contour map using the recorded FNET data is available on Youtube\footnote{\url{https://youtu.be/awvS4TtN77E}}. We have recovered the propagation time by observing how long  after the impulse start time the frequency overshoot with the highest red color has arrived at each location equipped with FNET devices. For example, in 1.7 seconds}, the frequency overshoot reached an intersected area among Arkansas, Tennessee, Kentucky and Missouri. In 2.7 seconds, the EM wave front reached the regions of North Dakota, Upstate New York and Massachusetts. \colorcode{Note that these recorded values may not be the ground-truth because of the observation error in the recovery process.} %because of the eye-balling method and the lack of exact peak location in the video. Nevertheless, those values are representative for electro-mechanical wave propagation property in the EI system.} %\footnote{\url{https://www.youtube.com/watch?v=awvS4TtN77E}}.


A sample of the ambient frequency data with its detrended output at a selected location is shown in Fig. \ref{fig:PMU}. The bandpass filter in [S2] was implemented using the function $fir1$ of Matlab$^\circledR$ at an order of 300 samples  with the lower and upper cutoff frequency at 0.075Hz and 1Hz, respectively. This high filter order can yield very low filter gain at low frequency regime and thus efficiently detrend the input data.

\begin{figure}
	\centering
	\begin{subfigure}{1\linewidth}
		\centering
		\epsfig{file = Figs/RealData/PMU1.eps, width = 0.92\textwidth}
	%	\subcaption{A sample PMU frequency measurement.}
		\label{fig:PMUa}
	\end{subfigure}
	\begin{subfigure}{1\linewidth}
		\centering
		\epsfig{file = Figs/RealData/PMU_filtered1.eps, width = 0.92\textwidth}
	%	\subcaption{The associated filtered PMU measurement.}
		\label{fig:PMUb}
	\end{subfigure}
	\caption{A sample of the raw ambient frequency measurement (top) and its corresponding detrended component (down).}
	\label{fig:PMU}
\end{figure}

We cross-correlate the detrended frequency data at the Florida location with every other location to determine the corresponding frequency response. Fig. \ref{fig:realdata} plots selected response from the FNET meter 623, at Florida, to meters 726, 781 and 823, at North Dakota, Missouri and Arkansas, respectively. The peak of each response is located at 2.4, 2.0 and 1.6 seconds, respectively. This is used to estimate the arrival time of EM oscillations and compared with the recorded values, as listed in Table \ref{tbl:RealData} for all locations. The recorded value is obtained from the replay video of this event. For the aforementioned three locations, the recorded value is 2.5, 2.1, and 1.5 seconds, respectively. Clearly, the cross-correlation approach has successfully estimated the propagation time from the source of disturbance to other location, with  the average error around 0.2 second.  

\colorcode{Various factors can attribute to the mismatch error between the recorded and estimated propagation time. First, the recorded values themselves may be different from the ground-truth propagation time. They have been recovered from the Youtube video showing frequency contour map and would suffer from some observation error. Second, the location of disturbance input is slightly different between the 2008 blackout and the 2017 ambient data. Due to limited deployment of FNET devices, the only frequency measurement available in Florida is located at Lakeland, about 250 miles north of the actual source of 2008 blackout, Turkey Point. Third, there is a fundamental limit in the estimated time resolution of 0.1 second as the ambient FNET data has a sampling frequency at 10 Hz. Last but not least, the blackout happened in 2008 while the ambient data was collected in 2017. Over the past  decade, significant changes have taken place in the EI grid. Nonetheless, extensive real data based studies in \cite{2017Cui_oscillationanalysis} have demonstrated that the statistics of inter-area oscillation modes and EM waves has stayed almost the same for the EI grid. Hence, we believe that the 2008 Florida blackout event can still serve as a good reference for validating our real data test. Meanwhile, the mismatch error at 0.2 second is consistent with the time resolution of 0.1 second, which has verified the effectiveness of our proposed approach.}

%}. First, the ideal conditions in (as1)-(as3) definitely fail to hold for the EI system. Hence, the modes are neither perfectly decoupled nor uniformly excited. \colorcode{Due to limited access to PMU measurements, the only available one in Florida is at Lakeland, 250 miles north of Turkey Point, the location of disturbance in the Florida Blackout. This spatial distance would add to the difference betwen the recorded and estimated propagation times}. Moreover, the frequency sampling rate at 10Hz would result in a limited time resolution of 0.1 second. Last, the event happened in 2008 but the ambient data was collected in 2017. In the last decade, changes have taken place in the EI grid, such as the types of generation. Nevertheless, the overall high fidelity between the recorded and estimation results may point out that the major inter-area modes have not changed very much for the EI grid. \colorcode{This hypothesis is also corroborated by \cite{2017Cui_oscillationanalysis}. Using FNET data, this paper shows the inter-area oscillation statistical properties of the EI system has not been altered significantly during the 2010-2017 period.}

\begin{figure}[tb!]
	\centering
	\epsfig{file = Figs/RealData/Xcor_selfig1.eps, width = 1\linewidth}		
	\caption{Cross-correlation of ambient frequency deviation for the pairs 623--726 (Florida -- North Dakota), 623--781 (Florida -- Missouri) and 623--823 (Florida -- Arkansas).}
	\label{fig:realdata}
\end{figure}

\begin{table}[tb!]
	\centering
	\caption{Recorded versus estimated propagation time}
	\label{tbl:RealData}
	\begin{tabular}{|c|c|c|c|}
		\hline
		Location      & Meter  & Recorded & Estimated \\ \hline
		Virginia      & 601     & 1.5  & 1.1  \\ \hline
		Alabama       & 671     & 0.7  & 0.4  \\ \hline
		Massachussets & 682     & 2.6  & 2.3  \\ \hline
		North Dakota  & 726     & 2.5  & 2.4  \\ \hline
		Missouri      & 756     & 1.6  & 1.9  \\ \hline
		Illinois      & 767     & 1.5  & 1.7  \\ \hline
		Missouri      & 781     & 2.1  & 2.0  \\ \hline
		Tennessee     & 787     & 1.6  & 1.5  \\ \hline
		Arkansas      & 823     & 1.5  & 1.6  \\ \hline
	\end{tabular}
\end{table}
